CoverBLIP: accelerated and scalable iterative matched-filtering for Magnetic Resonance Fingerprint reconstruction

Current popular methods for Magnetic Resonance Fingerprint (MRF) recovery are bottlenecked by the heavy computations of a matched-filtering step due to the growing size and complexity of the fingerprint dictionaries in multi-parametric quantitative MRI applications. We address this shortcoming by arranging dictionary atoms in the form of cover tree structures and adopt the corresponding fast approximate nearest neighbour searches to accelerate matched-filtering. For datasets belonging to smooth low-dimensional manifolds cover trees offer search complexities logarithmic in terms of data population. With this motivation we propose an iterative reconstruction algorithm, named CoverBLIP, to address large-size MRF problems where the fingerprint dictionary i.e. discrete manifold of Bloch responses, encodes several intrinsic NMR parameters. We study different forms of convergence for this algorithm and we show that provided with a notion of embedding, the inexact and non-convex iterations of CoverBLIP linearly convergence toward a near-global solution with the same order of accuracy as using exact brute-force searches. Our further examinations on both synthetic and real-world datasets and using different sampling strategies, indicates between 2 to 3 orders of magnitude reduction in total search computations. Cover trees are robust against the curse-of-dimensionality and therefore CoverBLIP provides a notion of scalability -- a consistent gain in time-accuracy performance-- for searching high-dimensional atoms which may not be easily preprocessed (i.e. for dimensionality reduction) due to the increasing degrees of non-linearities appearing in the emerging multi-parametric MRF dictionaries.

==> sections/mrf_part.tex <==
\section{Application in Quantitative MRI}


%The main body of measurements in MR imaging comes from the net magnetic moment of proton spins in a given voxel.
%Excitations in form of rotating the external magnetic field, referred to as Flip Angles (FAs), apply at certain time intervals. Proton spins respond to these excitations; they get aligned with the new field and yet, relax back to the equilibrium state however non-instantaneously. 
%Two exponents characterize the time proton magnetization takes to reach equilibrium: i) the \emph{spin-lattice} longitudinal relaxation $T1$, 
%%the exponent related to the time for longitudinal magnetization component to recover, 
%and ii) the \emph{spin-spin} transverse relaxation $T2$. These exponents are unique for biological tissues.

In \emph{quantitative MRI} 
%(in contrast with single image qualitative MRI) 
rather than simply forming a single MR image with only  contrast information (i.e. qualitative MRI), physicists
are interested in measuring the NMR properties of tissues   namely, the $T1,T2$ relaxation times, $\delta f$ magnetic resonance and proton density (PD), and use these parameters to differentiate different biological tissues~\cite{toftsqmri}. The standard approach for parameter estimation is to acquire a large sequence
of images in different times from a simple excitation pulse (i.e. excitations in terms of rotating the magnetic field)  and then use an exponential model curve fitting to recover the decay exponents $T1,T2$ for each voxel. This procedure runs separately to estimate each relaxation time.
The long process of acquiring multiple fully sampled images, brings serious limitation to standard approaches in quantitative imaging to apply within a reasonable time and with an acceptable signal-to-noise ratio (SNR) and resolution.
%
%These procedures are 
% \eqref{eq:mrf-decay1} and \eqref{eq:mrf-decay2} see for instance \nref [Wajiha's]. 
% 
%%which characterizes decay of the transversal component.
%More formally, for $\m(t)=[\m^x(t) \, \m^y(t) \, \m^z(t)]^T$ the magnetization vector at time $t$ we have:
%\begin{align}
%\m^z (t)&= \m^z_{eq} - \left(\m^z_{eq}-\m^z(0)\right)e^{-t/{T1}}, \label{eq:mrf-decay1}\\  
%\m^{xy}(t) &= \m^{xy}(0)e^{-t/{T2}}.\label{eq:mrf-decay2}
%\end{align}
%Interestingly, different molecular structures have distinct $T1,T2$ relaxations. For instance, it has been discovered in '70s that tumours have higher $T1$ relaxation times than normal tissues.
%%; a discovery which brings huge attention to such characterization since 1971. 
%Since then more studies have established relating certain neurological degradations (causing brain disorders e.g. MS) to anomalies observed in relaxation times, which ultimately established a whole field of study known as \emph{quantitative MRI}:
%Rather than simply forming a single MR image that measures
%the transverse magnetization response, physicists
%measure the NMR properties of tissue namely, $T1,T2$ and proton density (PD), and use these parameters to differentiate different biological tissues\nref [paul Toft book]. The standard approach for parameter estimation is to acquire a large sequence
%of images in different times from an initial excitation pulse, and then use exponential curve fitting to recover $T1,T2$ per voxel using models \eqref{eq:mrf-decay1} and \eqref{eq:mrf-decay2} see for instance \nref [Wajiha's]. 


\subsection{Magnetic Resonance Fingerprinting}



Recently, a novel parameter estimation process coined as the \emph{Magnetic Resonance Fingerprinting} (MRF) has been proposed to address this shortcoming. 
For the acquisition, MRF applies a shorter sequence of random excitations (i.e. $\Gamma \in [0,\pi/2]^{\n}$ random flip angels with  typically $\n\approx 300-1000$ and the time interval $TR\sim 10-40$ msec) for estimating all parameters $T1,T2,\delta f$, and proton density at once.
%\item This sequence can be further optimized and shortened w.r.t. the random choice of FAs, see \nref [Cohen'15, Mahbub'16].
 After each excitation pulse the response is recorded  through the 
measurements taken from a small portion of k-space.
%\end{itemize} 
As a result the acquisition time can significantly decreases to a couple of minutes \cite{MRF}.   

The exponential model as for the traditional acquisition sequences will no longer hold for the MRF model. Due to using random excitations, the signatures casts a non-trivial implicit expression  readable by solving the \emph{Bloch dynamic equations} $\Bb(\Gamma,\Theta)\in \CC^\n $ customized for the set of parameters $\Theta=\{T1,T2,\delta f\}$. 
The MRF problem is an example of data driven CS model with an algebraic signal model (i.e. the Bloch equations) but a non-trivial projection. For this problem one constructs off-line a
dictionary of \emph{fingerprints} (i.e. magnetization responses) for all possible $d=\#\{\Theta_i\}_i$ parameters presented in normal tissues where the atoms $\psi_i:=\Bb(\Gamma,\Theta_i)$ uniquely represent the underlying set of parameters $\Theta_i$ . This corresponds
to sampling a low-dimensional manifold associated with the
solutions of the Bloch dynamic equations~\cite{BLIPsiam}, which for complicated excitation patterns neither the response nor the projection has an
analytic solution.


%These signatures are calculated off-line for all possible $d=\#(\Theta)$ parameters and saved in a huge dictionary of \emph{fingerprints} whose atoms $\psi_i:=\Bb(\Gamma,\Theta_i)$ uniquely represent the underlying set of parameters $\Theta_i$. 


\subsection{MRF image model and parameter estimation}

%The underlying MRF image is a 3-dimensional tensor. By matricization 
An MRF image can be represented by a matrix $X\in \CC^{ \n\times J}$. Each column $X_j$ represents a $\n$-dimensional spatial pixel $j$ and each row $X^l$  represents a temporal image slice (with the spatial resolution equal to $J$) corresponding to the measurements taken after the excitation pulse $\Gamma_l$, $\forall l=1,\ldots,\n$. The total spatio-temporal resolution of the MRF image is $n:=\n J$. By the pixel purity assumption, the image follows the product space data driven model \eqref{eq:dmodel} and \eqref{eq:immodel} where each column/pixel $j$ correspond to a single fingerprint $\psi$ with a unique parameter  $\Theta$. The cone($\widetilde \Cc$) corresponds to the fingerprints dictionary and $\rho>0$ represents the proton density.\footnote{The proton density can be generally a complex number for which only the rescaling step of the cone projection slightly changes and the rest of the analysis similarly holds, for more details see~\cite{BLIPsiam}. %but here for simplicity we assume it to be a positive real number, although a similar analysis applies for the complex case~\cite{BLIPsiam}.
	} 
The MRF acquisition model is linear as follows:
\eql{\label{eq:CSMRF}	
	Y^l \approx \Ff_{\Omega_l} (X^l), \quad \forall l=1,\ldots \n,
}
where  $\Ff$ denotes the two-dimensional Fourier transform, and $\Ff_{\Omega_l}: \CC^J \rightarrow \CC^{m/\n}$ subsamples the k-space coefficients of the  image slice $X^l$ according a pattern/set $\Omega_l$.  The k-space subsampling could correspond to a spiral pattern~\cite{MRF} or a random horizontal/vertical line subselection~\cite{BLIPsiam} e.g. in the Echo Planar Imaging (EPI). %, from the 2-dimensional spatial Fourier domain.  
By vectorization of $X,Y$, we have a product space CS model similar to~\eqref{eq:CSsampling} for a sampling protocol $A$ acting spatially however with different k-space sampling pattern per image slice. 
%is $A=\Ff_{\Omega_i}\otimes I_J$ for $\otimes$ denoting the Kronecker product.

%Projection onto the Bloch manifold $\Bb$ is non-trivial for a random FA pattern (as neither the manifold nor and the projection are explicitly given). The MRF framework addresses this bottleneck with model discretezation of as explained in Section~\ref{sec:discrete}. One has to solve the Bloch equations for $d$ number of discretized parameters $\Theta$, and yet store the outcome Bloch response signature $\psi_j$ in a dictionary $\Psi$ corresponding to~\eqref{eq:discrete}. This is a preprocessing step and potentially can lead to a very large size dictionary with $d\sim O(10^6)$ atoms! Therefore in a sense the MRF framework sacrifices the memory in order to enable/facilitate the projection step of IPG.

The CS reconstruction proposed by~\cite{BLIPsiam} is based on a data driven IPG algorithm (with the \emph{exact} cone projection described in Section~\ref{sec:datadrivenCS}) where one by identifying the correct fingerprint per pixel $X_j$ can recover the underlying parameters $\Theta$ stored in a look-up table (the last rescaling step also recovers the proton density $\gamma_j$). 
It has been shown in~\cite[Theorem 1]{BLIPsiam} that if $\Omega_l$ independently at random subselects the rows (or columns) of the k-space, which corresponds to a \emph{random EPI sampling protocol}, the resulting forward map $A$ is bi-Lipschitz  w.r.t. the product model $\Cc=\prod_{j=1}^J \text{cone}(\widetilde \Cc)$, provided sufficient \emph{discriminations} between the fingerprints.\footnote{One achieves a suitable discrimination between the MR fingerprints by e.g. choosing the random excitation sequence long enough.} This result guarantees stability of the parameter estimation using this algorithm with an step size $\mu=n/m$.

Since the Bloch manifold is parametrized by only three parameters in $\Theta$ and thus has a low intrinsic dimension, we use the cover tree ANN searches to accelerate the projection step. We perform the following procedure iteratively until convergence:
\begin{align*}\label{eq:BLIP}
(X^l)^{k+1} = 
\Pp^{\epsilon}_{\text{cone}(\widetilde \Cc)} \left( (X^l)^{k} - \mu \Ff^H_{\Omega_l}\left(\Ff_{\Omega_i} ((X^l)^{k})  -Y^l\right) \right) 
\end{align*}
The approximate cone projection follows the update in~\eqref{eq:ANN1}. 


Provided with the same embedding result (for the random EPI acquisition protocol) and according to Theorem~\ref{th:inexactLS2} we can deduce the linear convergence of this algorithm to the true solution for mildly-chosen approximations $\epsilon$ (and the same step size $\mu=n/m$) where the projection step has now the complexity $O(J\log(d))$. For large-sized dictionaries the gap between the computation costs of the exact and  inexact IPG algorithm can be significantly large. %and a well-chosen step size e.g. $\mu \approx m/n$. And as consequence one achieves an exact parameter $\Theta$ estimation.



